Pricing Economic Dispatch with AC Power Flow via Local Multipliers and Conic Relaxation

We analyze pricing mechanisms in electricity markets with AC power flow equations that define a nonconvex feasible set for the economic dispatch problem. Specifically, we consider two possible pricing schemes. The first among these prices are derived from Lagrange multipliers that satisfy Karush-Kuhn-Tucker conditions for local optimality of the nonconvex market clearing problem. The second is derived from optimal dual multipliers of the convex semidefinite programming (SDP) based relaxation of the market clearing problem. Relationships between these prices, their revenue adequacy and market equilibrium properties are derived and compared. The SDP prices are shown to equal distribution locational marginal prices derived with second-order conic relaxations of power flow equations over radial distribution networks. We illustrate our theoretical findings through numerical experiments.

==> figure_1.tex <==

\begin{figure}[h]
	\centering
 	\vspace{-10pt}
	\subfloat[P.1][]{
		\includegraphics[trim=80pt 30pt 80pt 10pt ,clip, width=0.23\textwidth]{standard_real.png}
		\label{fig:bus30_standard.p}}
%
	\subfloat[Q.1][]{
		\includegraphics[trim=80pt 30pt 80pt 10pt ,clip, width=0.23\textwidth]{standard_reactive.png}
		\label{fig:bus30_standard.q}}
\\
\vspace{-10pt}
	\subfloat[P.2][]{
		\includegraphics[trim=80pt 30pt 80pt 10pt ,clip, width=0.23\textwidth]{real_case2.png}
		\label{fig:bus30_case2.p}}
%
	\subfloat[Q.2][]{
		\includegraphics[trim=80pt 30pt 80pt 10pt ,clip, width=0.23\textwidth]{reactive_case2.png}
		\label{fig:bus30_case2.q}}
\\
\vspace{-10pt}
	\subfloat[P.3][]{
		\includegraphics[trim=80pt 30pt 80pt 10pt ,clip, width=0.23\textwidth]{real_case3.png}
		\label{fig:bus30_case3.p}}
%
	\subfloat[Q.3][]{
		\includegraphics[trim=80pt 30pt 80pt 10pt ,clip, width=0.23\textwidth]{reactive_case3.png}
		\label{fig:bus30_case3.q}}
	\caption{Plots (a), (b) show heatmaps of SDP-LMPs on the 30-bus IEEE network. Plots (c), (d) are derived with $p_{26}^{D} =7.5$, $q_{26}^{D} =3.3$, $p_{29}^{D} =12.2 $, $q_{29}^{D} =4.9 $, $p_{30}^{D} = 16.1 $, and $q_{30}^{D} = 5.9$. Plots (e), (f) are derived with $\ul{v}_k = 0.99$, $\ol{v}_k = 1.01$ for $k=24,\ldots,30$. Prices in (a), (c), (f) are real power prices (in \$/MWh) and those in (b), (d), (f) are reactive power prices (in \$/MVARh).}
	\label{fig:heat_bus30}
	\vspace{-10pt}
\end{figure}



==> table.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table*}[t]
	\centering
	\begin{tabular}{c c c c c c c c c c c c c c  c } 
		\toprule
		Case &  $f$ & $r$ & $x$ & $k$ &
		$p_k^D$ & $q_k^D$ & $\ol{p}_k^G$ & $\ol{q}_k^G$ & $\ul{v}_k^2$ & $\ol{v}_k^2$ & $C^1_k$ & $C^2_k$ & $w_k^\star$ & MS \\ [0.5ex] 
		\midrule
		\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &1&0.79&0.50&2.0&0.90&0.95&0.98&10&1.0&0.98 & \multicolumn{1}{c}{}\\\multicolumn{1}{c}{\multirow{-1}{*}{1}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.24}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.01}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.01}} & 2&0&0&1.2&0.21&0.98&1.01&10&1.0&0.99&\multicolumn{1}{c}{\multirow{-1}{*}{-2.44}}\\\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &3&1.90&0&2.0&2.00&0.99&1.01&10&1.0&0.99 & \multicolumn{1}{c}{}
		\\
		\midrule
		\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &1&0.79&0.50&2.0&0.90&0.95&1.05&10&1.0&1.01 & \multicolumn{1}{c}{}\\\multicolumn{1}{c}{\multirow{-1}{*}{2}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.50}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.01}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.01}} & 2&0&0&1.2&0.21&0.98&1.01&10&1.0&1.01&\multicolumn{1}{c}{\multirow{-1}{*}{0.71}}\\\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &3&2.00&0&2.0&2.00&0.99&1.01&10&1.0&1.00 & \multicolumn{1}{c}{}\\ \midrule
		
		\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &1&0.79&0.50&2.0&0.90&1.01&1.05&10&1.0&1.01 & \multicolumn{1}{c}{}\\\multicolumn{1}{c}{\multirow{-1}{*}{3}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.50}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.01}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.01}} & 2&0&0&1.2&0.21&0.98&1.01&10&1.0&1.01&\multicolumn{1}{c}{\multirow{-1}{*}{0.17}}\\\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &3&2.00&0&2.0&2.00&0.99&1.01&10&1.0&1.00 & \multicolumn{1}{c}{}\\ 
\midrule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &1&1.10&1.00&1.0&2.0&0.98&1.01&10&0.1&1.01 & \multicolumn{1}{c}{}\\\multicolumn{1}{c}{\multirow{-1}{*}{4}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.90}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.03}} & \multicolumn{1}{c}{\multirow{-1}{*}{0.75}} & 2&1.10&1.00&3.0&2.0&0.99&1.01&1&0.1&1.01&\multicolumn{1}{c}{\multirow{-1}{*}{16.04}}\\\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &3&0.95&1.00&0&2.0&0.95&1.02&0&0&0.95 & \multicolumn{1}{c}{}\\ \bottomrule	

	\end{tabular}
	\caption{Parameter choices and outcomes of the case studies on the three-bus power network.}
	\vspace{-10pt}
	\label{tab:table1}
\end{table*}

